Weakly Supervised Grounding for VQA in Vision-Language Transformers

Transformers for visual-language representation learning have been getting a lot of interest and shown tremendous performance on visual question answering (VQA) and grounding. But most systems that show good performance of those tasks still rely on pre-trained object detectors during training, which limits their applicability to the object classes available for those detectors. To mitigate this limitation, the following paper focuses on the problem of weakly supervised grounding in context of visual question answering in transformers. The approach leverages capsules by grouping each visual token in the visual encoder and uses activations from language self-attention layers as a text-guided selection module to mask those capsules before they are forwarded to the next layer. We evaluate our approach on the challenging GQA as well as VQA-HAT dataset for VQA grounding. Our experiments show that: while removing the information of masked objects from standard transformer architectures leads to a significant drop in performance, the integration of capsules significantly improves the grounding ability of such systems and provides new state-of-the-art results compared to other approaches in the field.

==> fig3.tex <==
% \begin{figure}[t]

% \begin{tabular}{c}
% {
% \includegraphics[width=0.5\linewidth]{images/capsule_layer_v3.png}
% }
% % \subcaptionbox{Self Attention}{\includegraphics[width=0.23\linewidth]{images/self-attention.pdf}} &
% % \subcaptionbox{Cross-Self Attention}{\includegraphics[width=0.4\linewidth]{images/cross-self-attention.pdf}} 
% \end{tabular}
% % \vspace{-10pt}
%  \caption{Overview of the proposed capsule layer. Similar to the Capsule encoding, input tokens $X'$ are first transformed into capsules $X_c$. The output feature $h^i_{cls}$ corresponding to $[CLS]$ token from the text encoder layer $i$ learns the presence probability of a certain capsule at the layer $i$ in visual encoder. This mask $m^i$ selects the capsules respective to the attended words at text encoder layer $i$. The resulting capsules are then flattened and upsampled (denoted by $\hat{x}^i_{j_{mc}}$) and added to the output $h^{i-1}_{cls}$ of the previous visual transformer layer $i-1$ to obtain input features $\hat{h}^{i-1}_{v_j}$ for the next visual transformer layer $i$. }
% \label{fig:capsules-layer}
% \vspace{-5pt}
% \end{figure}

% %----------------------------------------------------------------------------------------

==> teaser.tex <==
%---------------------------------------------------------------------------------------------

\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
 \includegraphics[width=\linewidth]{images/teaser.pdf}

\end{center}
\vspace{-5pt}
  \caption{\textbf{ Attention from the proposed vision-language transformer with VQA supervision.} We look at the self-attention of the [IMG] token on the heads of the last layer. These maps show that the model automatically learns to ground relevant objects leading to weakly-supervised grounded VQA (GVQA). \textit{blue box is ground truth, orange is predicted box.}}
\vspace{-15pt}
\label{fig:teaser}
\end{figure}


%--------------------------------------------------------------------------------

